Verified System Development with the AutoFocus Tool Chain

This work presents a model-based development methodology for verified software systems as well as a tool support for it: an applied AutoFocus tool chain and its basic principles emphasizing the verification of the system under development as well as the check mechanisms we used to raise the level of confidence in the correctness of the implementation of the automatic generators.

==> eptcsdata.tex <==
\providecommand{\firstpage}{17}
\providecommand{\publicationstatus}{C. Andr\'es and L. Llana (Eds.): 2nd Workshop on Formal\\
Methods in the Development of Software 2012 (WS-FMDS 2012).\\
EPTCS 86, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.86.3}{10.4204/EPTCS.86.3}}
\pdfoutput=1

